Motion and Force Planning for Manipulating Heavy Objects by Pivoting

Manipulation of objects by exploiting their contact with the environment can enhance both the dexterity and payload capability of robotic manipulators. A common way to manipulate heavy objects beyond the payload capability of a robot is to use a sequence of pivoting motions, wherein, an object is moved while some contact points between the object and a support surface are kept fixed. The goal of this paper is to develop an algorithmic approach for automated plan generation for object manipulation with a sequence of pivoting motions. A plan for manipulating a heavy object consists of a sequence of joint angles of the manipulator, the corresponding object poses, as well as the joint torques required to move the object. The constraint of maintaining object contact with the ground during manipulation results in nonlinear constraints in the configuration space of the robot, which is challenging for motion planning algorithms. Exploiting the fact that pivoting motion corresponds to movements in a subgroup of the group of rigid body motions, SE(3), we present a novel task-space based planning approach for computing a motion plan for both the manipulator and the object while satisfying contact constraints. We also combine our motion planning algorithm with a grasping force synthesis algorithm to ensure that friction constraints at the contacts and actuator torque constraints are satisfied. We present simulation results with a dual-armed Baxter robot to demonstrate our approach.

==> preliminaries_old.tex <==
\section{Preliminaries}

\noindent
\textbf{Quaternions}: The quaternions are the set of hypercomplex numbers, $\mathbb{H}$. A quaternion $Q \in \mathbb{H}$ can be represented as $Q = q_0 + \boldsymbol{q} = q_0 + q_1 i + q_2 j + q_3 k$ or a 4-tuple $Q = (q_0, \boldsymbol{q}_r) = (q_0, q_1, q_2, q_3)$ where $\mathbb{H}$ is set of all quaternions, $q_0 \in \mathbb{R}$ is the real scalar part, $\boldsymbol{q}$ is the imaginary vector part,
% $\mathbb{R}$ is the real Euclidean space,
$\boldsymbol{q}_r=(q_1, q_2, q_3) \in \mathbb{R}^3$ is a real vector,
%$q_1, q_2, q_3 \in \mathbb{R}$,
and $i, j, k$ are quaternion units or imaginary orthogonal axes that obey Hamilton's rule $i^2=j^2=k^2=ijk=-1$.
% \orange{Quaternions can represent all scalars in $\mathbb{R}$ when
%$q_1=q_2=q_3=0$ $\boldsymbol{q}_r=\boldsymbol{0}$ and all vectors in $\mathbb{R}^3$ when $q_0=0$.}
The conjugate, norm, and inverse of the quaternion $Q$ is represented as
%$Q^* = q_0 - \boldsymbol{q}$
$Q^* = (q_0, -\boldsymbol{q}_r)$, $\lVert Q \rVert = \sqrt{Q Q^*} = \sqrt{Q^* Q}$,
%  = \sqrt{q_0^2 + q_1^2 + q_2^2 + q_3^2}
and $Q^{-1} = Q^*/{\lVert Q \rVert}^2$, respectively. Addition and multiplication of two quaternions
% $P = p_0 + \boldsymbol{p} =(p_0, \boldsymbol{p}_r)$
% $Q = q_0 + \boldsymbol{q} = (q_0, \boldsymbol{q}_r)$
$P = (p_0, \boldsymbol{p}_r)$ and
$Q = (q_0, \boldsymbol{q}_r)$ are performed as $P+Q = (p_0 + q_0, \boldsymbol{p}_r + \boldsymbol{q}_r)$ and $PQ = (p_0 q_0 - \boldsymbol{p}_r \cdot \boldsymbol{q}_r, p_0 \boldsymbol{q}_r + q_0 \boldsymbol{p}_r + \boldsymbol{p}_r \times \boldsymbol{q}_r)$.
% \orange{As a result, $PQ \ne QP$, $(PQ)^* = Q^* P^*$, $\lVert PQ \rVert = \lVert P \rVert \lVert Q \rVert$, and $QQ^{-1}=Q^{-1}Q=1$.}
The quaternion $Q$ is a \textit{unit quaternion}
% or \textit{versor}
if ${\lVert Q \rVert} = 1$, and consequently, $Q^{-1} = Q^*$.

\noindent
\textbf{Dual Quaternions}:
In general, dual numbers are defined as $d = a + \epsilon b$ where $a$ and $b$ are elements of an algebraic field, and $\epsilon$ is a \textit{dual unit} with $\epsilon ^ 2 = 0, \epsilon \ne 0$.
%\orange{Moreover, a function $f(a + \epsilon b)$ can be expanded using the Taylor expansion as $f(a)+\epsilon bf'(a)$.}
Similarly, a dual quaternion $D$ is defined as $D= P + \epsilon Q$
% or an 8-tuple $D=(P, Q)$
where $P, Q \in \mathbb{H}$. The conjugate, norm, and inverse of the dual quaternion $D$ is represented as $D^* = P^* + \epsilon Q^*$, $\lVert D \rVert = \sqrt{D D^*} = \sqrt{P P^* + \epsilon (PQ^* + QP^*)}$, and $D^{-1} = D^*/{\lVert D \rVert}^2$,
% = P^{-1} (1-\epsilon QP^{-1})
respectively. Another definition for the conjugate of $D$ is represented as $D^\dag = P^* - \epsilon Q^*$. Addition and multiplication of two dual quaternions $D_1= P_1 + \epsilon Q_1$ and $D_2= P_2 + \epsilon Q_2$ are performed as $D_1 + D_2 = (P_1 + P_2) + \epsilon (Q_1 + Q_2)$ and $D_1 D_2 = (P_1 P_2) + \epsilon (P_1 Q_2 + Q_1 P_2) $.
% \orange{As a result, $D_1 D_2 \ne D_2 D_1$, $(D_1 D_2)^* = D_2^* D_1^*$, $(D_1 D_2)^\dag = D_2^\dag D_1^\dag$, and $DD^{-1}=D^{-1}D=1$.}
The dual quaternion $D$ is a \textit{unit dual quaternion} if ${\lVert D \rVert} = 1$, i.e., ${\lVert P \rVert} = 1$ and $PQ^* + QP^* = 0$, and consequently, $D^{-1} = D^*$.


\noindent
\textbf{Rigid-Body Motion}: The rigid-body motion is represented by the relative motion of a body-fixed coordinate frame $\{b\}$ with respect to an inertia/base coordinate frame $\{s\}$. Thus, the rigid-body motion (i.e., rotation $\boldsymbol{R} \in SO(3)$ and translation $\boldsymbol{p} \in \mathbb{R}^3$) can be described by the pair $(\boldsymbol{R},\boldsymbol{p})$ or the Special Euclidean group $SE(3)=SO(3) \times \mathbb{R}^3$ where $SO(3) \subset \mathbb{R}^{3 \times 3}$ is the Special Orthogonal group representing the space of all rigid-body rotations. Mathematically, $SO(3)=\left\{\boldsymbol{R} \in \mathbb{R}^{3 \times 3}\left|\boldsymbol{R}^{\mathrm{T}} \boldsymbol{R}=\boldsymbol{R} \boldsymbol{R}^{\boldsymbol{T}}=\boldsymbol{I}_3,\right| \boldsymbol{R} \mid=1\right\}$ and $S E(3)=\left\{(\boldsymbol{R}, \boldsymbol{p}) \mid \boldsymbol{R} \in S O(3), \boldsymbol{p} \in \mathbb{R}^{3}\right\}$ where $\boldsymbol{I}_3$ is a $3\times3$ identity matrix and $\left| \cdot \right|$ is the determinant operator. An element $\boldsymbol{T} \in SE(3)$, which is a pose of the rigid body, can be expressed by a $4 \times 4$ homogeneous transformation matrix as
$\boldsymbol{T} = \left[\begin{smallmatrix}\boldsymbol{R}&\boldsymbol{p}\\\boldsymbol{0}&1\end{smallmatrix}\right]$ where $\boldsymbol{0}$ is a $1 \times 3$ zero vector.
% $T = \left[\begin{array}{ll} \boldsymbol{R} & \boldsymbol{p} \\ \boldsymbol{0}_{1\times 3} & 1 \end{array}\right]$.
The rotation $\boldsymbol{R} \in SO(3)$ represented by rotation of an angle $\theta \in [0,\pi]$ about a unit axis $\boldsymbol{l} \in \mathbb{R}^3$ can be also expressed by a unit quaternion as $Q_R = (\cos\frac{\theta}{2}, \boldsymbol{l} \sin\frac{\theta}{2}) \in \mathbb{H}$.
% Consequently, if we first apply the rotation $Q_{R1} \in \mathbb{H}$, and then the rotation $Q_{R2} \in \mathbb{H}$, the resulting rotation is $Q_{R1}Q_{R2}$.
Moreover, the rotation of a point or vector $\boldsymbol{v} \in \mathbb{R}^3$ by the angle $\theta$ about an axis in the direction $\boldsymbol{l}$ through the origin is determined as $Q_{v'} = Q_R Q_v Q_R^*$ where $Q_v = (0,\boldsymbol{v}) \in \mathbb{H}$. A power of $Q_R$ is also defined as $Q_R^\tau = (\cos\frac{\tau\theta}{2}, \boldsymbol{l} \sin\frac{\tau\theta}{2})$. The homogeneous transformation $\boldsymbol{T} \in SE(3)$ (i.e., the rotation $\boldsymbol{R}$ followed by the translation $\boldsymbol{p}$) can be also represented by a unit dual quaternion as $D_T = Q_R + \frac{\epsilon}{2} Q_p Q_R$ where $Q_p = (0, \boldsymbol{p}) \in \mathbb{H}$. Consequently, for the pure rotation and pure translation, the transformation $D_T$ is $Q_R + \epsilon 0$ and $1 + \frac{\epsilon}{2} Q_p$, respectively. The transformation of a point or vector $\boldsymbol{v} \in \mathbb{R}^3$ is determined as $D_T(1+\epsilon Q_v)D_T^\dag = 1+\epsilon(Q_RQ_vQ_R^*+Q_p)$. Based on Chasles-Mozzi theorem \cite{ModernRobotics_LynchPark2017}, all rigid-body transformations can also be expressed as a screw displacement. 

\noindent
\textbf{Screw Displacement}: Chasles-Mozzi theorem states that the general Euclidean displacement/motion of a rigid body in 3-dimensional Euclidean space from the origin $\boldsymbol{I}$ to $\boldsymbol{T} = (\boldsymbol{R},\boldsymbol{p}) \in SE(3)$
can be expressed as rotation $\theta$ about a fixed axis $\mathcal{S}$, called the \textit{screw axis}, and a translation $d$ along that axis as shown in Fig.~\ref{Fig:ScrewDisplacement}. Plücker coordinates can be used to represent the screw axis by $\boldsymbol{l}$ and $\boldsymbol{m}$, where $\boldsymbol{l} \in \mathbb{R}^3$ is a unit vector that represents the direction of the screw axis $\mathcal{S}$, $\boldsymbol{m} = \boldsymbol{r} \times \boldsymbol{l}$, and $\boldsymbol{r} \in \mathbb{R}^3$ is an arbitrary point on the axis. Thus, the screw parameters are define as $\boldsymbol{l}, \boldsymbol{m}, \theta, d$.
% and the pitch of the screw displacement is $\theta/d$.
The screw displacements can be expressed by the dual quaternions as $D_T = Q_R + \frac{\epsilon}{2} Q_p Q_R = (\cos \frac{\Phi}{2}, L \sin \frac{\Phi}{2})$ where $\Phi = \theta + \epsilon d$ is a dual number and $L = \boldsymbol{l} + \epsilon \boldsymbol{m}$ is a
% unit
dual vector.
% with zero scalar part.
A power of the dual quaternion $D_T$ is then defined as $D_T^{\tau} = (\cos \frac{\tau \Phi}{2}, L \sin \frac{\tau \Phi}{2})$, $\tau >0$.
% Note that axis $L$ is independent of $\tau$.

% $D_T = Q_R + \epsilon Q_p Q_R/2 = \cos \frac{\Theta}{2} + L \sin \frac{\Theta}{2}$
% $D_T^{\tau} = \cos \frac{\tau \Theta}{2} + L \sin \frac{\tau \Theta}{2}$ 

\begin{figure}[!htbp]
    \centering
    \includegraphics[scale=0.51]{Figures/ScrewDisplacement.pdf}
    \caption{Screw displacement from pose $\mathcal{C}_1$ to pose $\mathcal{C}_2$.}
\label{Fig:ScrewDisplacement}
\end{figure}

\noindent
\textbf{Screw Linear Interpolation (ScLERP)}: To perform a one degree-of-freedom smooth screw motion (with a constant rotation and translation rate) between two object poses in $SE(3)$, the screw linear interpolation (ScLERP) can be used. The ScLERP provides a \textit{straight line} in $SE(3)$ which is the closest path between two given poses in $SE(3)$. However, note that the origin of the object does not necessarily follow a straight line in
% the real Euclidean space
$\mathbb{R}^3$.
% If the poses are represented by $4 \times 4$ homogeneous transformation matrices $\boldsymbol{T}_1$ and $\boldsymbol{T}_2$, the path provided by the ScLERP is derived by $\boldsymbol{T}(\tau)=\boldsymbol{T}_{1} \exp \left(\log \left(\boldsymbol{T}_{1}^{-1} \boldsymbol{T}_{2}\right) \tau \right)$ where $ \tau \in[0,1]$ is a scalar path parameter, $\exp(\cdot)$ is matrix exponential, and $\log(\cdot)$ is matrix logarithm. Similarly,
If the poses are represented by unit dual quaternions $D_{1}$ and $D_{2}$, the path provided by the ScLERP is derived by $D(\tau) = D_1 (D_1^{-1}D_2)^{\tau}$ where $ \tau \in[0,1]$ is a scalar path parameter and $D_{12} = D_1^{-1}D_2 = D_1^{*}D_2$ represents the pose $D_2$ relative to the pose $D_1$ (or the transformation from $D_1$ to $D_2$). As $\tau$ increases from 0 to 1, the object moves between two poses along the path
% $\boldsymbol{T}(\tau)$ or
$D(\tau)$ (which is a straight line in $SE(3)$) by the rotation $\tau \theta$ and translation $\tau d$. In order to find $D_{12}^\tau$, the screw coordinates $\boldsymbol{l}, \boldsymbol{m}, \theta, d$ are first extracted from $D_{12} = P + \epsilon Q = (p_0,\boldsymbol{p}_r) + \epsilon (q_0,\boldsymbol{q}_r) = (\cos\frac{\theta}{2}, \boldsymbol{l} \sin\frac{\theta}{2}) + \epsilon Q$ by $\boldsymbol{l} = \boldsymbol{p}_r/ \lVert \boldsymbol{p}_r \lVert $, $\theta = 2 \, \mathrm{atan2}(\lVert \boldsymbol{p}_r \lVert, p_0)$, $d = \boldsymbol{p} \cdot \boldsymbol{l}$, and $\boldsymbol{m} = \frac{1}{2} (\boldsymbol{p} \times \boldsymbol{l} + (\boldsymbol{p}-d \boldsymbol{l})\cot \frac{\theta}{2})$ where $\boldsymbol{p}$ is derived from $2QP^* = (0, \boldsymbol{p})$ and $\mathrm{atan2}(\cdot)$ is the two-argument arctangent. Then, $D_{12}^\tau = (\cos \frac{\tau \Phi}{2}, L \sin \frac{\tau \Phi}{2})$ is directly derived from $\left(\cos \frac{\tau \theta}{2}, \sin \frac{\tau \theta}{2}\boldsymbol{l}\right)+\epsilon \left( -\frac{\tau d}{2}\sin \frac{\tau \theta}{2}, \frac{\tau d}{2}\cos \frac{\tau \theta}{2}\boldsymbol{l}+\sin \frac{\tau \theta}{2}\boldsymbol{m} \right) $. Note that $\theta =0, \pi$ corresponds to pure translation between two poses and the screw axis is at infinity.
